StructChart: On the Schema, Metric, and Augmentation for Visual Chart Understanding

Charts are common in literature across various scientific fields, conveying rich information easily accessible to readers. Current chart-related tasks focus on either chart perception that extracts information from the visual charts, or chart reasoning given the extracted data, e.g. in a tabular form. In this paper, we introduce StructChart, a novel framework that leverages Structured Triplet Representations (STR) to achieve a unified and label-efficient approach to chart perception and reasoning tasks, which is generally applicable to different downstream tasks, beyond the question-answering task as specifically studied in peer works. Specifically, StructChart first reformulates the chart data from the tubular form (linearized CSV) to STR, which can friendlily reduce the task gap between chart perception and reasoning. We then propose a Structuring Chart-oriented Representation Metric (SCRM) to quantitatively evaluate the chart perception task performance. To augment the training, we further explore the potential of Large Language Models (LLMs) to enhance the diversity in both chart visual style and statistical information. Extensive experiments on various chart-related tasks demonstrate the effectiveness and potential of a unified chart perception-reasoning paradigm to push the frontier of chart understanding.

==> section/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/xiarenqiu.jpg}}]{Renqiu Xia}
is currently a Ph.D. candidate at the School of Electronic Information and Electrical Engineering, Shanghai Jiao Tong University, under the supervision of Prof. Junchi Yan. His primary research interests encompass Neural Architecture Search and Multi-modal Large Language Models, with a particular focus on document understanding and mathematical reasoning. Additionally, he regularly serves as a reviewer for CVPR, KDD and TKDE.
\end{IEEEbiography}


\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/phy.jpg}}]{Haoyang Peng}
received his Master's degree in Electronic Engineering from the School of Information Science and Technology, Fudan University, Shanghai, China, in 2024. His research interests include few-shot learning, weakly-supervised learning, and vision-language models in document understanding.
\end{IEEEbiography}

\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/yhc.jpg}}]{Hancheng Ye}
received his B.S. and M.S. degrees in Electronic Engineering at School of Information Science and Technology from Fudan University. He is currently a research assistant at Shanghai Artificial Intelligence Laboratory. His primary research interests focus on efficient machine learning, model compression, and multimodal learning.
\end{IEEEbiography}

\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/lms.png}}]{Mingsheng Li} received the B.S. degree in Electronic Engineering from Fudan University, Shanghai, China, in 2022, where he is currently pursuing the M.S. degree with the School of Information Science and Technology. His long-term research interests include computer vision, multi-modal learning, and vision-and-language. 
\end{IEEEbiography}

\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/yxc.jpg}}]{Xiangchao Yan}
recieved M.S. degree from Shanghai Jiao Tong University. He is currently an algorithm researcher at Shanghai Artificial Intelligence Laboratory. His research interests include generalized representation learning in 3D scenes, 3D scene pre-training, and multi-modal document understanding.
\end{IEEEbiography}

\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/yp.jpg}}]{Peng Ye}
is currently a postdoctoral fellow at mmlab of the Chinese University of Hong Kong. He received his Ph.D. degree at Fudan University, Shanghai, China. His research interests include computer vision, network design, and optimization. He has published papers in leading journals and conferences including PAMI, IJCV, CVPR Oral, ICCV, ECCV, NeurIPS Spotlight, ICML, ACM MM Oral, ICME Best Student Paper, TGRS, TCSVT, etc. 
% He serves as a  reviewer in kinds of journals and conferences including TPAMI, IJCV,CVPR, ECCV, ICCV, NIPS etc.
\end{IEEEbiography}

\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/sbt.jpg}}]{Botian Shi}
received the Ph.D. degree from the School of Computer Science \& Technology, Beijing Institute of Technology, China, in 2021. He is currently a Researcher at ADLab of Shanghai Artificial Intelligence Laboratory, Shanghai, China. His research interests include Autonomous Driving Systems, Embodied Artificial Intelligence as well as Knowledge-driven Autonomous Driving.
\end{IEEEbiography}

\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/qy.jpeg}}]{Yu Qiao} (Senior Member, IEEE) received the Ph.D. degree from The University of Electro-Communications, Japan, in 2006.
He now is the lead scientist at Shanghai AI Laboratory, a researcher, and the honored director of the Multimedia Laboratory at Shenzhen Institutes of Advanced Technology at the Chinese Academy of Sciences (SIAT).
He served as an assistant professor at the Graduate School of Information Science and Technology at the University of Tokyo from 2009 to 2010. He has been working on deep learning since 2006, and he is one of the earliest people to introduce deep learning to video understanding. He and his team invented center loss and temporal segment networks. He has published more than 400 articles in top-tier conferences and journals and conferences in computer science with more than 60,000 citations. He received the CVPR 2023 Best Paper Award and AAAI 2021 Outstanding Paper Award. His research interests revolve around foundation models, computer vision, deep learning, robotics, and AI applications.
\end{IEEEbiography}

\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/yjc}}]{Junchi Yan} (Senior Member, IEEE) is the Deputy Director and Professor with School of Artificial Intelligence and Department of Computer Science and Engineering, Shanghai Jiao Tong University (SJTU), Shanghai, China. Before that, he was a Research Staff Member with IBM Research where he started his career since April 2011 and until 2018. He obtained his Ph.D. in Electronic Engineering with SJTU in 2015. He received the Best Paper Candidate of CVPR 2024. His research interests include machine learning and applications. He regularly serves as Senior PC/Area Chair for NeurIPS, ICML, ICLR, CVPR, AAAI, IJCAI, SIGKDD, and Associate Editor for IEEE TPAMI, Pattern Recognition. He is a Fellow of IAPR.
\end{IEEEbiography}

\vspace{-12mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/zb.jpg}}]{Bo Zhang} is currently a Research Scientist at the Shanghai Artificial Intelligence Laboratory. His work has garnered numerous awards, including the Shanghai Rising Star from the Shanghai Municipal Commission of Science and Technology, and the National Scholarship 2021 China Award. He has published 22 papers in top-tier international conferences and journals such as CVPR, ICLR, NeurIPS, T-PAMI, TIP, and IJCV. He also serves as a reviewer for several prestigious academic conferences and journals, including CVPR, ECCV, ICCV, ICLR, and ICML. Professionally, he led the development of the 3DTrans general scene representation open-source project, which won the Waymo Challenge international competition and accumulated over 7.5K stars. Additionally, he is committed to promoting the rapid application of multi-modal large language models in various scenarios, such as scientific document understanding, scientific research surveys, mathematical reasoning, and autonomous driving.
\end{IEEEbiography}

==> tables/1-related.tex <==
\begin{table*}[tb!]
\centering
\caption{\small Comparisons of different research works on chart data, where CP, CR, and CU represent the chart perception, chart reasoning, and chart understanding works, respectively. S. and R. denote the summarization and redrawing tasks, respectively.}
\small
\scalebox{0.95}{
\begin{tabular}{c|l|ccc|ccc|ccc|cc|ccc}
\toprule
&\multirow{2}{*}{Methods} & \multicolumn{3}{c}{Chart Types} & &\multirow{2}{*}{Perception} & & Reasoning / & &\multicolumn{2}{c}{Perception}  & &\multicolumn{3}{c}{Downstream Tasks}         \\ 
\cline{3-5} \cline{11-12} \cline{14-16}
&  & Line & Bar & Pie& & &&  Understanding && \multicolumn{1}{c}{Format} & Metric & & QA & S. & R.  \\ \hline
\multirow{5}{*}{\rotatebox[origin=b]{90}{\textbf{CP}}} & ReVision~\cite{Savva2011ReVisionAC}& & \checkmark &\checkmark & &\checkmark & & \multirow{5}{*}{\fontsize{30.0pt}{\baselineskip}\selectfont $\ \backslash$ } & & \multicolumn{1}{c}{\multirow{5}{*}{JSON}}& & & \multicolumn{3}{c}{\multirow{5}{*}{\fontsize{35.0pt}{\baselineskip}\selectfont $\ \backslash$ }}  \\
& ChartReader~\cite{Rane2021ChartReaderAP}  & & \checkmark & & & \multicolumn{1}{c}{\checkmark} & &  &  & & \multicolumn{1}{c}{Component}  &  & &  \\
& \cite{Liu2019DataEF} & & \checkmark & & & \multicolumn{1}{c}{\checkmark} & & & & & \multicolumn{1}{c}{-level} & &  &  \\
& \cite{Choi2019VisualizingFT} & & & \multicolumn{1}{c}{\checkmark} & & \multicolumn{1}{c}{\checkmark}  & & & & & & &  \\
\cline{12-12}
& ChartOCR~\cite{Luo2021ChartOCRDE}   & \checkmark & \checkmark  & \multicolumn{1}{c}{\checkmark} & & \multicolumn{1}{c}{\checkmark} & & & & & \multicolumn{1}{c}{Type-level} & &  & &  \\ \hline
% \multirow{4}{*}{\rotatebox[origin=b]{90}{\textbf{CR}}}  & T5-OCR~\cite{Masry2022ChartQAAB}  & \checkmark  & \checkmark & \multicolumn{1}{c|}{\checkmark} &\multicolumn{1}{c|}{\checkmark}  & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\multirow{4}{*}{LCT} }  & \multirow{4}{*}{\fontsize{30.0pt}{\baselineskip}\selectfont $\backslash$} & \checkmark&  & \\
% & TaPas-OCR~\cite{Masry2022ChartQAAB} & \checkmark & \checkmark   & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark}  &\multicolumn{1}{c|}{\checkmark}  &\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}  & \checkmark  &  &   \\
% & VL-T5-OCR~\cite{Masry2022ChartQAAB}   & \checkmark  & \checkmark  & \multicolumn{1}{c|}{\checkmark}& \multicolumn{1}{c|}{\checkmark} &\multicolumn{1}{c|}{\checkmark} &\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \checkmark & & \\
% & VisionTaPas-OCR~\cite{Masry2022ChartQAAB} & \checkmark & \checkmark & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} &\multicolumn{1}{c|}{\checkmark} &\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}  & \checkmark & &  \\ \hline
% %\cline{8-8}
% %& Pix2Struct~\cite{Lee2022Pix2StructSP} & \checkmark  & \checkmark  & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{\checkmark} &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \checkmark & &  \\ \hline
% \multirow{3}{*}{\rotatebox[origin=b]{90}{\textbf{CU}}} & Matcha~\cite{Liu2022MatChaEV}  & \checkmark  & \checkmark & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\textbf{--}}  & \multicolumn{1}{c|}{\checkmark}   &\multicolumn{1}{c|}{\textbf{--}}   & \multicolumn{1}{c|}{\textbf{--}}  & \checkmark  & \checkmark  & \\
% %\cline{8-8}
% & Deplot~\cite{Liu2022DePlotOV} & \checkmark   & \checkmark & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark}&\multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{LCT}  &\multicolumn{1}{c|}{\textbf{--}}   & \checkmark & \checkmark  & \\
% \cline{2-12} 
% & StructChart (Ours)  & \checkmark  & \checkmark  & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark}&\multicolumn{1}{c|}{\checkmark}  & \multicolumn{1}{c|}{STR}  & \multicolumn{1}{c|}{SCRM} & \checkmark  & \checkmark & \checkmark \\ \hline
\end{tabular}
}
\label{tab:rw_compare}
\end{table*}

==> tables/3-sim-se-old.tex <==
\begin{table*}[!tb]
\centering
\caption{\small ChartQA perception results by scaling up the simulation data (from 0.1K to 9K).}
% \vspace{-6pt}
\scalebox{0.95}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ccrccccccccccc}
\toprule

\qquad \qquad &\multirow{2}*{Train Set} & $IoU_{thr}$ $\rightarrow$ &  &\multicolumn{2}{c} {mPrecision} & & \multicolumn{4}{c} {Precision} & \\ \cmidrule{5-6} \cmidrule{8-12}
& & Tolerance $\downarrow$ & & \multicolumn{2}{c} {0.5:0.05:0.95} &  &0.5& 0.75 & 0.95 & 1 (EM) \\
\midrule

& \multirow{3}*{\begin{tabular}{c}
      ChartQA\\
     (w/o sim data)  
 \end{tabular}}  
& strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & &\multicolumn{2}{c}{0.6770} & &0.7273 &0.6714 &0.6458 &0.6326 &\\
& & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.7792} & &0.8220&0.7746 &0.7519 &- &\\
& & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.8274} & &0.8703 &0.8210 &0.8011 &- &\\

\midrule 
 % \rowcolor{applegreen!20}
 \multirow{14}{*}{\rotatebox[origin=b]{90}{ Real \& Simulated Source}}
 & \multirow{3}*{\begin{tabular}{c}
      ChartQA\\
     +SimChart0.1K  
 \end{tabular}}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.6804} & &0.7282 &0.6752 &0.6468 &0.6383 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.7893} & &0.8305 &0.7850 &0.7595 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.8326} & &0.8731 &0.8277 &0.8087 &-&\\ \cmidrule{2-12}

 & \multirow{3}*{\begin{tabular}{c}
      ChartQA\\
     +SimChart1K  
 \end{tabular}}
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.6871} &&0.7367 &0.6828 &0.6544 &0.6458 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.7938} &&0.8371 &0.7907 &0.7661 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.8394} &&0.8788 &0.8362 &0.8116 &- &\\ \cmidrule{2-12}

 % & \multirow{3}*{ChartQA+SimChart 3k}  
 % & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.6952} &&0.7434 &0.6913 & 0.6913 &0.6506 &\\
 % & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.7986 } &&0.8428 &0.7964  &0.7699 &- &\\
 % & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.8366} &&0.8807 &0.8333 &0.8068 &- &\\ \cmidrule{2-12}

 & \multirow{3}*{\begin{tabular}{c}
      ChartQA\\
     +SimChart6K  
 \end{tabular}}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.7040} &&0.7491  &0.7036 &0.6686 &0.6591 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.8128} &&0.8580  &0.8116 &0.7794 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.8450 } &&0.8835  &0.8428 &0.8182 &- &\\ \cmidrule{2-12}

 & \multirow{3}*{\begin{tabular}{c}
      ChartQA \\
      +SimChart9K
 \end{tabular}
}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.7116} &&0.7595 &0.7074 &0.6809 &\textbf{0.6686} &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.8182} &&0.8674 &0.8144 &0.7850 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{\textbf{0.8527}} &&\textbf{0.8958} &\textbf{0.8532} &\textbf{0.8220} &- &\\
\bottomrule 
\end{tabular}
}
\label{tab:sim}
% \vspace{-2pt}
\end{table*}

==> tables/4-fewshot-old.tex <==
\begin{table*}[tb!]
\centering
\caption{\small Zero-shot and few-shot on real-world chart dataset by means of the proposed SimChart9K.}
% \vspace{-6pt}
\scalebox{0.95}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{ccrccccccccccc}
\toprule
\qquad &\multirow{2}*{Train Set} & $IoU_{thr}$ $\rightarrow$ &  &\multicolumn{2}{c} {mPrecision} & & \multicolumn{4}{c} {Precision} & \\ \cmidrule{5-6} \cmidrule{8-12}
& & Tolerance $\downarrow$ & & \multicolumn{2}{c} {0.5:0.05:0.95} &  &0.5& 0.75 & 0.95 & 1 (EM) \\
\midrule
 \multirow{14}{*}{\rotatebox[origin=b]{90}{No Simulated Source}}
 & \multirow{3}*{ChartQA0.01}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.1797} &&0.2121 &0.1771 &0.1591 &0.1534 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.2384} &&0.2850 &0.2339 &0.2178 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.2686} &&0.3277 &0.2633 &0.2424 &-&\\ \cmidrule{2-12}
 & \multirow{3}*{ChartQA0.1}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.3616} &&0.4015 &0.3598 &0.3277 &0.3210 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.4242} &&0.4612 &0.4195 &0.4025 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.4653} &&0.5038 &0.4631 &0.4422 &-&\\ \cmidrule{2-12}
  & \multirow{3}*{ChartQA0.5}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.5389} &&0.5786 &0.5350 &0.5085 &0.4981 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.6150} &&0.6525 &0.6089 &0.5890 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.6603} &&0.6951 &0.6553 &0.6392 &-&\\  \cmidrule{2-12}
& \multirow{3}*{ChartQA}  
& strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & &\multicolumn{2}{c}{0.6770} & &0.7273 &0.6714 &0.6458 &0.6326 &\\
& & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.7792} & &0.8220&0.7746 &0.7519 &- &\\
& & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.8274} & &0.8703 &0.8210 &0.8011 &- &\\
\midrule 
 % \rowcolor{applegreen!20}
 \multirow{2}{*}{\rotatebox[origin=b]{90}{Zero-shot}}
 & \multirow{3}*{SimChart9K}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.0688} &&0.0890 &0.0691 &0.0483 &0.0483 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.1577} &&0.1979 &0.1562 &0.1288 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.2527} &&0.3021 &0.2491 &0.2235 &-&\\ 
\midrule 
 % \rowcolor{applegreen!20}
 \multirow{12}{*}{\rotatebox[origin=b]{90}{Few-shot}}
 & \multirow{3}*{\begin{tabular}{c}
      ChartQA0.01\\
     +SimChart9K  
 \end{tabular}}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.3074} &&0.3797 &0.3078 &0.2500 &0.2348 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.4672} &&0.5227 &0.4706 &0.4138 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.5402} &&0.5909 &0.5398 &0.4981 &-&\\ \cmidrule{2-12}
 & \multirow{3}*{\begin{tabular}{c}
      ChartQA0.1\\
     +SimChart9K  
 \end{tabular}}  
 & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.5973} &&0.6619 &0.6013 &0.5483 &0.5294 &\\
 & & slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.7466} &&0.7936 &0.7500 &0.7112 &- &\\
 & & high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.7980} &&0.8419 &0.8002 &0.7661 &-&\\ \cmidrule{2-12}
 &\cellcolor{gray!10}&\cellcolor{gray!10} strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} &  \cellcolor{gray!10} &  \multicolumn{2}{c}{ \cellcolor{gray!10} 0.6465} & \cellcolor{gray!10}& \cellcolor{gray!10}0.7055 & \cellcolor{gray!10}0.6468 & \cellcolor{gray!10}0.5956 & \cellcolor{gray!10}0.5814 &\cellcolor{gray!10}\\
 &\cellcolor{gray!10} & \cellcolor{gray!10} slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} &\cellcolor{gray!10} & \multicolumn{2}{c}{\cellcolor{gray!10}0.7787} &\cellcolor{gray!10}&\cellcolor{gray!10}0.8229 &\cellcolor{gray!10}0.7775 &\cellcolor{gray!10}0.7443 &\cellcolor{gray!10}-&\cellcolor{gray!10} \\
 &\multirow{-3}*{\cellcolor{gray!10}\begin{tabular}{c}
      ChartQA0.2\\
     +SimChart9K  
 \end{tabular}}& \cellcolor{gray!10} high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} &\cellcolor{gray!10} &  \multicolumn{2}{c}{\cellcolor{gray!10}0.8206} &\cellcolor{gray!10}&\cellcolor{gray!10}0.8646 &\cellcolor{gray!10}0.8201 &\cellcolor{gray!10}0.7888 &\cellcolor{gray!10}-&\cellcolor{gray!10}\\ \cmidrule{2-12}
 &\cellcolor{gray!10} & \cellcolor{gray!10} strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} &\cellcolor{gray!10} & \multicolumn{2}{c}{\cellcolor{gray!10} 0.6902} &\cellcolor{gray!10}&\cellcolor{gray!10}0.7434&\cellcolor{gray!10}0.6913 &\cellcolor{gray!10}0.6487 &\cellcolor{gray!10}0.6420 &\cellcolor{gray!10}\\
 &\cellcolor{gray!10} & \cellcolor{gray!10} slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} &\cellcolor{gray!10} & \multicolumn{2}{c}{\cellcolor{gray!10}0.8015} &\cellcolor{gray!10}&\cellcolor{gray!10}0.8466 &\cellcolor{gray!10}0.8002 &\cellcolor{gray!10}0.7642 &\cellcolor{gray!10}- &\cellcolor{gray!10}\\
 & \multirow{-3}*{\cellcolor{gray!10}\begin{tabular}{c}
      ChartQA0.5\\
     +SimChart9K  
 \end{tabular}}   & \cellcolor{gray!10} high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} &\cellcolor{gray!10} &  \multicolumn{2}{c}{\cellcolor{gray!10}0.8380} &\cellcolor{gray!10}&\cellcolor{gray!10}0.8788 &\cellcolor{gray!10}0.8400 &\cellcolor{gray!10}0.8040 &\cellcolor{gray!10}-&\cellcolor{gray!10}\\ 
\bottomrule 
\end{tabular}
}
\label{tab:few-shot}
% \vspace{-8pt}
\end{table*}

==> tables/5-generalization.tex <==
% \begin{table}[H]
\centering
\caption{\small Generalizability study for few-shot on PlotQA and Chart2Text by means of SimChart9K.}
% \vspace{-6pt}
\scalebox{0.95}{
\renewcommand{\arraystretch}{1}
\begin{tabular}{cccrccccccccc}
\toprule

&\multirow{2}*{Val Set}  & \multirow{2}*{Train Set} 
& $IoU_{thr}$$\rightarrow$ &  &\multicolumn{2}{c} {mPrecision} & & \multicolumn{4}{c} {Precision} & \\ \cmidrule{6-7} \cmidrule{9-13}
& & &Tolerance $\downarrow$ & & \multicolumn{2}{c} {0.5:0.05:0.95} &  &0.5& 0.75 & 0.95 & 1 (EM) \\
\midrule

& \multirow{6}{*}{\rotatebox[origin=b]{90}{PlotQA}}
 &\multirow{3}*{PlotQA} & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & &\multicolumn{2}{c}{0.1995} &&0.2500 &0.1931 &0.1765 &0.1736 &\\
& &  &slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.7848} &&0.8519 &0.7784 &0.7405 &- &\\
& &  &high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.8271} &&0.8922 &0.8223 &0.7861 &- &\\  \cmidrule{3-13}

& &\multirow{3}*{\begin{tabular}{c}
      PlotQA0.1\\
     +SimChart9K  
 \end{tabular}} & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & &\multicolumn{2}{c}{0.1887} &&0.2452 &0.1874 &0.1684 &0.1612 &\\
& & &slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.7976} &&0.6624 &0.7948 &0.7517 &- &\\
& & &high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.8063} &&0.8689 &0.8033 &0.7614 &- &\\

\midrule

& \multirow{6}{*}{\rotatebox[origin=b]{90}{Chart2Text}}
 &\multirow{3}*{Chart2Text} & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & &\multicolumn{2}{c}{0.1936} &&0.2473 &0.1892 &0.1533 &0.1442 &\\
& & &slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.5524} &&0.6603 &0.5529 &0.4672 &- &\\
& & &high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.6945} &&0.7676 &0.6934 &0.6356 &- &\\ \cmidrule{3-13}

& &\multirow{3}*{\begin{tabular}{c}
      Chart2Text0.2\\
     +SimChart9K  
 \end{tabular}} & strict \ \textcolor{red!60}{\rule{0.5em}{0.5em}} & &\multicolumn{2}{c}{0.2610} &&0.3177 &0.2601 &0.2248 &0.1729 &\\
& & &slight\ \textcolor{yellow!60}{\rule{0.5em}{0.5em}} & & \multicolumn{2}{c}{0.5711} &&0.6731 &0.5698 &0.4872 &- &\\
& & &high \ \textcolor{green!60}{\rule{0.5em}{0.5em}} & &  \multicolumn{2}{c}{0.6871} &&0.7512 &0.6855 &0.6309 &- &\\

\bottomrule 
\end{tabular}
}
\label{tab:few-shot-rebuttal}
% \end{table}

==> tables/7-figureqa.tex <==
\begin{table}[!tb]
\centering
\captionof{table}{\small QA results on FigureQA. The exact Match (EM) metric is employed for evaluation.}
% \vspace{-6pt}
\centering
\scalebox{0.9}{
\begin{tabular}{llcccccccccccc}
\toprule
&\multirow{2}*{Model} &\multirow{2}*{Train Set \ }
& \multirow{2}*{FigureQA val}  \\    
& & &\\
\midrule
  \multirow{2}{*}{\textbf{Baseline} } 
& MatCha~\cite{Liu2022MatChaEV} & ChartQA/PlotQA/C.D. & 61.2 &  \\
& Deplot~\cite{Liu2022DePlotOV}+GPT-3.5 & ChartQA/PlotQA/C.D. & 53.9  \\
\midrule
\multirow{1}{*}{\textbf{STR}}
&StructChart+GPT3.5&Real\&Sim Merging &\textbf{63.3}   \\
\bottomrule 
\end{tabular}
}
\label{tab:figure_qa}
\end{table}

==> tables/chartqa-ori.tex <==
\begin{table*}[t]
\caption{\small QA results on ChartQA, where LCT and our STR are two different text representation formats. Exact Match (EM) metric is employed for evaluation.}
% \vspace{-6pt}
\centering
% \scalebox{0.98}{
\begin{tabular}{llcccccccccccccccc}
\toprule
&\multirow{2}*{Model} &\multirow{2}*{Train Set \ }
& \multicolumn{3}{c}{ChartQA val} & & \multicolumn{3}{c}{ChartQA test} \\  \cmidrule{4-6} \cmidrule{8-10}    
& & & aug. \textcolor{blue!30}{\rule{0.7em}{0.55em}} & human \textcolor{red!30}{\rule{0.7em}{0.55em}} & avg. & & aug. \textcolor{blue!30}{\rule{0.7em}{0.55em}} & human \textcolor{red!30}{\rule{0.7em}{0.55em}} & avg. \\

\midrule
  \multirow{6}{*}{\rotatebox[origin=c]{90}{ \textbf{Baseline} }} 
& VL-T5-OCR~\cite{Masry2022ChartQAAB}  &ChartQA & - & - & 41.6 & & - & - & -&\\
& Tapas-OCR~\cite{Masry2022ChartQAAB} &ChartQA& - & - & 45.5 & & - & - & -&\\ 
& PaLI-17B~\cite{Chen2022PaLIAJ} &ChartQA& 64.9 & 30.4 & 47.6 & & - & - & - &\\ 
& Pix2Struct~\cite{Lee2022Pix2StructSP} &ChartQA & 81.6 & 30.5 & 56.0 & & - & - & - & \\ 
& MatCha~\cite{Liu2022MatChaEV} & ChartQA/PlotQA/C.D. & 90.2  & 38.2 & 64.2 & & - & - & - & \\
& Deplot~\cite{Liu2022DePlotOV} & ChartQA/PlotQA/C.D. & 69.3  & 36.6 & 52.9 & & - & - & - & \\
\midrule 

 \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{LCT}}}
 &StructChart+Llama-13b &ChartQA+SimChart9K &68.2 &36.4 &52.3 & & & & &   \\
 &StructChart+Vicuna-13b &ChartQA+SimChart9K &69.1 &37.4 &53.3 & & & & & \\ 
 &StructChart+Llama3.1-8b &ChartQA+SimChart9K & & & & &74.0 &37.4 &55.7 & \\
 &StructChart+Llama3.1-70b &ChartQA+SimChart9K &83.2 &58.9 &71.1 & &90.8 &57.9 &74.3& \\
 &StructChart+GPT-4 &ChartQA+SimChart9K &84.1 &63.1 &73.6 & &91.9 &61.8 &76.8\\
 \cmidrule{2-10}
 &\multirow{4}*{StructChart+GPT3.5}
 &ChartQA &64.2 &37.1 &50.7 &    \\
& & Real Merging &69.9 &39.1 &54.5 &    \\
& &ChartQA0.2+SimChart9K &62.6 &36.0 &49.3 &    \\
& &ChartQA+SimChart9K &71.3 &41.2 &56.3 &    \\

\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{STR}}}
 &StructChart+Llama-13b &ChartQA+SimChart9K &71.2 &38.2 &54.7 & & & &    \\
 &StructChart+Vicuna-13b &ChartQA+SimChart9K &73.5 &39.4 &56.5 &  & & &   \\ 
 &StructChart+Llama3.1-8b &ChartQA+SimChart9K & & & & &78.3 &54.4 &66.4 \\
 &StructChart+Llama3.1-70b &ChartQA+SimChart9K &84.9 &60.6 &72.8 & &92.2 &59.3 &75.4 \\
 &StructChart+GPT-4 &ChartQA+SimChart9K &85.6 &64.5 &75.5 & &93.5 &63.5 &78.5\\
 \cmidrule{2-10}
&\multirow{4}*{StructChart+GPT3.5}
&ChartQA &78.5 &42.8 &60.7 &    \\
& &Real Merging &80.2 &44.3 &62.2 &    \\
& &ChartQA0.2+SimChart9K &76.3 &40.7 &58.5 &    \\
& &ChartQA+SimChart9K &\textbf{83.9} &\textbf{46.7} & \textbf{65.3}&    \\
\bottomrule 
\end{tabular}
% }
\label{tab:qa}
\end{table*}

==> tables/prompt.tex <==
\begin{table*}[tb!]
    \centering
    \small
    \renewcommand\tabcolsep{4pt} % Adjust column space
    \caption{Prompts of label-efficient chart simulation process by PlotAgent including (1) data simulation stage for labels generation. (2) image simulation stage for chart generation.}
    \label{fig:simulation_2}
    % \resizebox{0.9\textwidth}{!}{  % Resize the table to fit within the text width
    \begin{tabular}{c|p{12cm}}  % Use 12cm or adjust column width accordingly
     \toprule
     \textbf{Stage} & \textbf{Prompt}\\
     \midrule
    \textit{Data Simulation}  & 
     \begin{minipage}[t]{\textwidth}  % Auto-adjust minipage width
     \textbf{System Prompt:} Copying the following table information can be expanded and adapted as\\
     appropriate, The imitation is as irrelevant as possible to the original text.\\
     
    \textbf{Input Data}: The data is \texttt{<data> \{data\_LCT\} </data>}
     \end{minipage}
     \\
     \midrule
    \textit{Image Simulation}  & 
     \begin{minipage}[t]{\textwidth}  % Auto-adjust minipage width
     \textbf{System Prompt:}      
            Consider you are a professional Python grapher.\\
            Please draw and save a chart based on the following data using Python, and images must be \\
            clear and intuitive.\\  
            Choose a plot type that best suits the value, for example, line, column, scatter, and pie charts.\\ 
            Drawing techniques such as background grids can be used.\\
            Draw as much variety as possible.\\
            Clear the current image state at the end of the code.\\
            If the text length of the label is too long, use the method of adding the parameter \texttt{rotation}\\
            or display label on separate lines seting \texttt{wrap=true}.\\
            The figsize parameter is set to a larger setting to prevent content from being displayed. \\
            Automatically resize the image by \texttt{tight\_layout()}.\\
            You must use xticks to prevent interpolation.\\
            Do not set special fonts such as sans-serif and Arial etc. to avoid the problem of missing fonts.\\
            If the string in the picture is too long, find a way for all characters to show and not be\\
            overwritten and stacked on top of each other.\\
            Do not have extra leading words at the beginning and end of the generated code, such as\\
            \texttt{python code, python, ```}, etc.\\
            Check the generated code without errors, do not include undefined functions.\\

    \textbf{Data:}The data is \texttt{<data> \{data generated in previous stage\} </data>}
    \end{minipage}
    \\
    \bottomrule
    \end{tabular}
    % }  % End of resizebox
\end{table*}
